Using Unsupervised Learning to Explore Robot-Pedestrian Interactions in Urban Environments

This study identifies a gap in data-driven approaches to robot-centric pedestrian interactions and proposes a corresponding pipeline. The pipeline utilizes unsupervised learning techniques to identify patterns in interaction data of urban environments, specifically focusing on conflict scenarios. Analyzed features include the robot's and pedestrian's speed and contextual parameters such as proximity to intersections. They are extracted and reduced in dimensionality using Principal Component Analysis (PCA). Finally, K-means clustering is employed to uncover underlying patterns in the interaction data. A use case application of the pipeline is presented, utilizing real-world robot mission data from a mid-sized German city. The results indicate the need for enriching interaction representations with contextual information to enable fine-grained analysis and reasoning. Nevertheless, they also highlight the need for expanding the data set and incorporating additional contextual factors to enhance the robots situational awareness and interaction quality.

==> figures/tikz/pipeline.tex <==
\begin{tikzpicture}[
    >=stealth,
    node distance=2.2cm,
    database/.style={
      cylinder,
      minimum width = 1.5cm,
      minimum height = 1.3cm,
      cylinder uses custom fill,
      cylinder body fill=yellow!50,
      cylinder end fill=yellow!50,
      shape border rotate=90,
      aspect=0.55,
      draw
    }
  ]
  \tikzstyle{every node}=[font=\footnotesize]
    \node[database] (STATIC_CONTEXT_DB) at (0,0) {};
    \node at (STATIC_CONTEXT_DB) [text width=1.5cm, align=center] {Static context parameter};
    \node[database,right of=STATIC_CONTEXT_DB, xshift=0.3cm, cylinder body fill=gray!50,
    cylinder end fill=gray!50] (DYNAMIC_CONTEXT_PARAMETER_DB) {};
    \node at (DYNAMIC_CONTEXT_PARAMETER_DB) [text width=1.5cm, align=center] {Dynamic context parameter};
    \node[database,right of=DYNAMIC_CONTEXT_PARAMETER_DB, xshift=0.3cm] (HUMAN_BEHAVIOR_DB) {};
    \node at (HUMAN_BEHAVIOR_DB) [text width=1.8cm, align=center] {Human behavior};
    \node[database,right of=HUMAN_BEHAVIOR_DB, xshift=0.3cm] (ROBOT_BEHAVIOR_DB) {};
    \node at (ROBOT_BEHAVIOR_DB) [text width=1.6cm, align=center] {Robot behavior};
    \node[database,right of=ROBOT_BEHAVIOR_DB, xshift=0.3cm, cylinder body fill=gray!50,
    cylinder end fill=gray!50] (SUPERVISOR_DB) {};
    \node at (SUPERVISOR_DB) [text width=1.8cm, align=center] {Supervisor inputs};
    \node[database,right of=SUPERVISOR_DB, xshift=0.3cm, cylinder body fill=gray!50,
    cylinder end fill=gray!50] (WEATHER_DB) {};
    \node at (WEATHER_DB) [text width=1.8cm, align=center] {Weather conditions};

    \node at (STATIC_CONTEXT_DB.70) (START_SCP) {} ;
    \node at (STATIC_CONTEXT_DB.110) (START_SCP_OSM) {} ;
    \node at (HUMAN_BEHAVIOR_DB.north) [yshift=2cm, xshift=1.3cm] (CROSSING) {};
    \node at (CROSSING) [yshift=1cm] (START_ROS)  {};

    % OSM Path
    \draw [<-] (START_SCP_OSM) -- (START_SCP_OSM|-START_ROS) node [] {Open Street Map};
    \node at (CROSSING-|START_SCP_OSM) [anchor=south east, text width=2cm, align=right] () {OSM json file};
    \node at ($(CROSSING-|START_SCP_OSM) + (0.05,-0.1)$) [anchor=north east, text width=2cm, align=right] () {Road type\\Geo references};

    % ROS Path
    \node at (START_ROS) [] () {Recorded robot missions};
    \draw [->] (START_ROS) -- (CROSSING.center) -- (CROSSING.center -| START_SCP) -- (START_SCP);
    \draw [->] (CROSSING.center -| DYNAMIC_CONTEXT_PARAMETER_DB) -- (DYNAMIC_CONTEXT_PARAMETER_DB);
    \draw [->] (CROSSING.center -| HUMAN_BEHAVIOR_DB) -- (HUMAN_BEHAVIOR_DB.north);
    \draw [->] (CROSSING.center) -- (CROSSING.center -| ROBOT_BEHAVIOR_DB) -- (ROBOT_BEHAVIOR_DB);
    \draw [->] (CROSSING.center) -- (CROSSING.center -| SUPERVISOR_DB) -- (SUPERVISOR_DB);

    \tikzstyle{ParameterStyle}=[anchor=north west, text width=2cm, align=left]
    \node at ($(CROSSING-|START_SCP) + (0.05,-0.1)$) [ParameterStyle] () {Road type\\ Track width\\ House exists\\ Infrastructure\\ ...};
    \node at ($(CROSSING-|DYNAMIC_CONTEXT_PARAMETER_DB) + (0.05,-0.1)$) [ParameterStyle] () {Parked cars\\Billboards\\Bicycles\\other Pedestrians\\ ...};
    \node at ($(CROSSING-|HUMAN_BEHAVIOR_DB) + (0.05,-0.1)$) [ParameterStyle] () {...};
    \node at ($(CROSSING-|ROBOT_BEHAVIOR_DB) + (0.05,-0.1)$) [ParameterStyle] () {Movement state\\Position};
    \node at ($(CROSSING-|SUPERVISOR_DB) + (0.05,-0.1)$) [ParameterStyle] () {Speed control\\emergency stop};

    \node at (CROSSING) [anchor=south west] () {ROS2 Bag files};

    % Weather Path
    \draw [<-] (WEATHER_DB) -- (WEATHER_DB|-START_ROS)  node [] {Weather records};
    \node at (CROSSING-|WEATHER_DB) [anchor=south west] () {};
    \node at ($(CROSSING-|WEATHER_DB) + (0.05,-0.1)$) [ParameterStyle] () {Wind\\Rainfall\\Light conditions};

    % Analysis Path
    \node at ($(HUMAN_BEHAVIOR_DB)!0.5!(ROBOT_BEHAVIOR_DB) + (0,-1.8)$) [draw, minimum width=4cm, minimum height=0.8cm, fill=yellow!50](INTERACTION_EXTR) {Interaction abstraction};
    \draw[->] (HUMAN_BEHAVIOR_DB.south) -- (INTERACTION_EXTR.north -| HUMAN_BEHAVIOR_DB);
    \draw[->] (ROBOT_BEHAVIOR_DB.south) -- (INTERACTION_EXTR.north -| ROBOT_BEHAVIOR_DB);

    \node at ($(INTERACTION_EXTR) + (0,-1.5)$) [draw, minimum width=4cm, text width=4cm, align=center, minimum height=0.8cm, fill=yellow!50](CLUSTERING) {Scenario specific interaction clustering};
    \draw[->] (STATIC_CONTEXT_DB.south) -- (CLUSTERING.185 -| STATIC_CONTEXT_DB) -- (CLUSTERING.185);
    \draw[->] (DYNAMIC_CONTEXT_PARAMETER_DB.south) -- (CLUSTERING.175 -| DYNAMIC_CONTEXT_PARAMETER_DB) -- (CLUSTERING.175);
    \draw[->] (WEATHER_DB.south) -- (CLUSTERING.east -| WEATHER_DB) -- (CLUSTERING.east);
    \draw[->] (INTERACTION_EXTR.south) -- (CLUSTERING.north);

    \node at ($(CLUSTERING) + (0,-1.5)$) [draw, minimum width=4cm, text width=4cm, align=center, minimum height=0.8cm,fill=gray!50](EVALUATION) {Cluster evaluation};
    \draw[->] (SUPERVISOR_DB.south) -- (EVALUATION.east -| SUPERVISOR_DB) -- (EVALUATION.east);
    \draw[->] (CLUSTERING.south) -- (EVALUATION.north);

  \end{tikzpicture}

==> sections/table.tex <==
\begin{tikzpicture}
    \node (TABLE) {%
    \begin{tabular}{|l|l|llll|}
    \hline
    \textbf{Category} & \textbf{Subcategory}              & \multicolumn{4}{l|}{\textbf{Options}}                                                                                                                           \\ \hline
    \rowcolor[HTML]{C0C0C0} 
    \multicolumn{2}{|l|}{Abstract Conflict Situation}                                              & \multicolumn{1}{l|}{\color{red}Head on}                    & \multicolumn{1}{l|}{Crossing}                    & \multicolumn{1}{l|}{Overtaking}               &            \\ \hline
    Traffic           & Human count                       & \multicolumn{2}{l|}{individual person (\color{red}89\%)}          & \multicolumn{2}{l|}{group (\color{red}89\%)}                      \\ \cline{2-6} 
                      & Bicycle                          & \multicolumn{1}{l|}{none (\color{red}92\%)  }                       & \multicolumn{1}{l|}{pushing (\color{red}2\%)  }                     & \multicolumn{1}{l|}{riding (\color{red}6\%)  }                   &            \\ \cline{2-6} 
                      & Carriage                          & \multicolumn{1}{l|}{none}                       & \multicolumn{1}{l|}{baby carriage}               & \multicolumn{1}{l|}{shopping cart}            &            \\ \cline{2-6} 
                      & Aids for people with disabilities & \multicolumn{1}{l|}{none}                       & \multicolumn{1}{l|}{rollator}                    & \multicolumn{1}{l|}{wheel chair}              &            \\ \hline
    Environment       & Light conditions                  & \multicolumn{1}{l|}{Daylight}                   & \multicolumn{1}{l|}{Night}                       & \multicolumn{1}{l|}{}                         &            \\ \cline{2-6} 
                      & Rain                              & \multicolumn{1}{l|}{none}                       & \multicolumn{1}{l|}{light}                       & \multicolumn{1}{l|}{heavy}                    &            \\ \cline{2-6} 
                      & ...                               & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                         &            \\ \cline{2-6} 
                      & other pedestrians involved        & \multicolumn{1}{l|}{no}                         & \multicolumn{1}{l|}{yes}                         & \multicolumn{1}{l|}{}                         &            \\ \hline
    Track             & Junction                          & \multicolumn{1}{l|}{no}                         & \multicolumn{1}{l|}{yes}                         & \multicolumn{1}{l|}{}                         &            \\ \cline{2-6} 
                      & House exit                        & \multicolumn{1}{l|}{no}                         & \multicolumn{1}{l|}{yes}                         & \multicolumn{1}{l|}{}                         &            \\ \cline{2-6} 
                      & Shape                             & \multicolumn{1}{l|}{straight}                   & \multicolumn{1}{l|}{curved}                      & \multicolumn{1}{l|}{tight curve}              &            \\ \cline{2-6} 
                      & Surface                           & \multicolumn{1}{l|}{asphalt}                    & \multicolumn{1}{l|}{cobblestone}                 & \multicolumn{1}{l|}{unpaved}                  &            \\ \cline{2-6} 
                      & Width                             & \multicolumn{1}{l|}{robot width}                & \multicolumn{1}{l|}{2 x robot width}             & \multicolumn{1}{l|}{3 x robot width}          & open space \\ \cline{2-6} 
                      & ...                               & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                         &            \\ \hline
    \rowcolor[HTML]{C0C0C0} 
    Result            & actual collision                  & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}no} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}yes} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}} &            \\ \cline{2-6} 
    \rowcolor[HTML]{C0C0C0} 
                      & Human stopped movement            & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}no} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}yes} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}} &            \\ \cline{2-6} 
    \rowcolor[HTML]{C0C0C0} 
                      & Human changed direction           & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}no} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}yes} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}} &            \\ \cline{2-6} 
    \rowcolor[HTML]{C0C0C0} 
                      & ...                               & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}} &            \\ \hline
    \end{tabular}
    };
    
    %\draw[step=1cm,red,very thin] (-8,-4) grid (8,4);
    
    %\draw [red, very thick](0,3) -- (0, 2.5);
    
    \end{tikzpicture}
